RIAV-MVS: Recurrent-Indexing an Asymmetric Volume for Multi-View Stereo

This paper presents a learning-based method for multi-view depth estimation from posed images. Our core idea is a "learning-to-optimize" paradigm that iteratively indexes a plane-sweeping cost volume and regresses the depth map via a convolutional Gated Recurrent Unit (GRU). Since the cost volume plays a paramount role in encoding the multi-view geometry, we aim to improve its construction both at pixel- and frame- levels. At the pixel level, we propose to break the symmetry of the Siamese network (which is typically used in MVS to extract image features) by introducing a transformer block to the reference image (but not to the source images). Such an asymmetric volume allows the network to extract global features from the reference image to predict its depth map. Given potential inaccuracies in the poses between reference and source images, we propose to incorporate a residual pose network to correct the relative poses. This essentially rectifies the cost volume at the frame level. We conduct extensive experiments on real-world MVS datasets and show that our method achieves state-of-the-art performance in terms of both within-dataset evaluation and cross-dataset generalization. Code available: https://github.com/oppo-us-research/riav-mvs.

==> approach.tex <==
Our learning-based online MVS system inspired by \cite{liu2019neural} aims to predict depth maps %(with no temporal delay) 
%% there is some delay since we use a few future frames after the reference;
%in a sequential manner from the input image sequences or monocular videos, 
from monocular videos by processing the frames in sequence, denoted by $\mathbf{I}_{1}^{N} =\{I_1, I_2, \dots, I_N \}$. As shown in Figure \ref{mvs-fig:frame-seq}, a local time window $\mathcal{N}_{t} = [t-\delta{t}, ... , t, ..., t+\delta{t}]$ containing several nearby frames is considered. A network $\mathcal{F}_{\theta}$ is %learned 
trained to estimate depth maps $\hat{\mathbf{D}}_{t}$ as close as possible to the ground truth depth maps $\mathbf{D}_t$, with the camera intrinsic matrix $\mathbf{K}_t$ and camera poses $\mathbf{T}_t = [\mathbf{R}_t | \mathbf{c}_t ]$ (with rotation matrix $\mathbf{R}_t$ and translation $\mathbf{c}_t$) for time $t \in \mathcal{N}_{t}$ considered known. The learning problem is formulated as

%%having access to intrinsics and extrinsics doe not enable depth estimation. You also need the images. You should say that camera parameters and poses are considered known.

\begin{equation}\label{eq:online_mvs}
\hat{\mathbf{D}}_{t} = \mathcal{F}_{\theta}(\mathbf{I}_{t-\delta{t}}^{t+\delta{t}}, \mathbf{T}_{t-\delta{t}}^{t+\delta{t}}, \mathbf{K}_{t-\delta{t}}^{t+\delta{t}}
)
\end{equation}

\noindent where $\theta$ is a collection of learnable parameters. The notation $(\cdot)_{t-\delta{t}}^{t+\delta{t}}$ represents a set of samples corresponding to the local time window $\mathcal{N}_{t}$, \eg, $\mathbf{T}_{t-\delta{t}}^{t+\delta{t}} = \{ T_k | k \in \mathcal{N}_{t} \}$ is a set of camera poses.

\begin{figure*}[!htbp]
    \centering
    \renewcommand{\tabcolsep}{1pt}
    \scriptsize
    %\includegraphics[width=0.95\textwidth]{ imgs-\imgres{}/frame-seq-2.png}
    \includegraphics[width=0.9\textwidth]{imgs-high-res/local-time-window.png}
    \caption{\textbf{An input video stream contains a sequence of frames $S_{1}^{N} =\{I_1, I_2, \dots, I_N \} $.} The depth is estimated for the reference frame $I_t$ by considering a local time window of several neighboring frames $\mathcal{N}_t = [t-\delta{t}, ... , t, ..., t+\delta{t}]$. %with $I_t$ as the reference frame. 
    Iteratively, as more frames become available, the next local time window $\mathcal{N}_{t+1}$ is processed with $I_{t+1}$ as a new reference frame.}
    %\vspace{-4pt}
    \label{mvs-fig:frame-seq}
\end{figure*}

Our approach is discussed in two sections. Sec. \ref{nrgbd-backbone} shows a backbone network based on the one by Liu \etal \cite{liu2019neural}, % (network based on the one by Liu et al." ----- let's give credit here)
which is %named %(name --> refer to)
referred to as NRGBD in this %paper 
chapter for convenience. As shown in Fig. \ref{mvs-fig:archi-backbone}, it consists of three parts, including i) the D-Net, which estimates the Depth Probability Volume (DPV) for each input frame, ii) the K-Net, which integrates the DPVs over time, and iii) the R-Net, which improves the spatial resolution of DPVs with the guidance from input images. Sec. \ref{depth-guided-dpv-update} presents our approach that integrates depth information between successive frames over time by Gaussian modulation and dynamic filtering, \cf Fig. \ref{mvs-fig:archi-ours}.


\begin{figure*}[!htbp]
    \centering
    \renewcommand{\tabcolsep}{1pt}
    \scriptsize
    \includegraphics[width=\textwidth]{ imgs-\imgres/backbone-nrgbd.png}
    \caption{\textbf{Architecture of Backbone network NRGBD \cite{liu2019neural}}. It includes D-Net for depth probability volume (DPV) construction, K-Net to integrate the DPV over time, and R-Net to refine and upsample the DPV to the spatial resolution of input frames.}
    \label{mvs-fig:archi-backbone}
    %\vspace{-8pt}
\end{figure*}






\subsection{DPV-based Backbone MVS Network} \label{nrgbd-backbone}

This section illustrates the backbone network, including two variants: i) NRGBD \cite{liu2019neural} and ii) a modified version by replacing its D-Net with a lightweight structure from MVSNet \cite{yao2018mvsnet}. \cf Fig. \ref{mvs-fig:archi-backbone}. The model function $\mathcal{F}_{\theta}$ in Eq. \ref{eq:online_mvs} is implemented by setting $\delta{t} = 2$, i.e., it takes an intrinsic matrix and a reference image at time $t$, four source images from time $t-2$, $t-1$, $t+1$ and $t+2$, and their corresponding poses and intrinsics. $\mathcal{F}_{\theta}$ predicts a depth map for the reference frame $I_{t}$. The backbone structure consists of three main parts.

%\subsubsection{DPV Construction}
\noindent \textbf{DPV Construction.} \,\, The depth probability volume (DPV) is defined on the 3D view frustum attached to the camera in perspective projection. It is generated by employing the traditional plane-sweep stereo \cite{space-sweep-collins, gallup2007real}, with $M = 64$ plane hypotheses, each parameterized by its depth $d$ that is uniformly sampled in the depth space, i.e., $ d \sim U(d_{\text{min}}, d_{\text{max}})$. Here $d_{\text{min}}$ and $d_{\text{max}}$ are the near and far planes of the 3D frustum, respectively. The DPV is denoted as $p(d; (u, v))$, or in short $p(d)$ by omitting $(u, v)$ for simplicity, being the probability of pixel $(u, v)$ having a depth value $d$. Specifically, for a given depth hypothesis and the reference frame $I_t$, a cost map is computed by i) warping all the neighboring frames in $\mathcal{N}_{t}$ into the current frame $I_t$ and ii) calculating the sum of $L_2$ or $L_1$ distances between the reference feature map and the warped feature maps. This way, we can construct a cost volume for all depth candidates, and further produce the DPV via feeding the cost volume to a \textit{softmax} layer $\sigma(\cdot)$. It is formulated in Eq. \ref{eq:dpv}:

\begin{equation}\label{eq:dpv}
%%too long for cvpr paper
%\mathbf{p}(d_t | I_t; \mathbf{I}_{t-\delta{t}}^{t+\delta{t}}, \mathbf{T}_{t-\delta{t}}^{t+\delta{t}}, \mathbf{K}_{t-\delta{t}}^{t+\delta{t}}) = \sigma \left( \sum_{k \in \mathcal{N}_{t}, k \neq t} \| f(I_t) - \mathbf{H}_2(f(I_k); d_t, T_{k}, T_{t}, K_{k}, K_{t})\| \right)
\mathbf{p}(d_t | I_t) = \sigma \left( \sum_{k \in \mathcal{N}_{t}, k \neq t} \| f(I_t) - \mathbf{H}_2(f(I_k); d_t \| \right)
\end{equation}



\noindent where $f(\cdot)$ is a subnetwork for deep feature extraction, and $\mathbf{H}_2(\cdot)$ is a 2D homography \cite{gallup2007real} that warps the image features from a source frame $I_k$ to the reference frame $I_t$. In this chapter, %paper, 
the subscript $k$ is used for %("is for" --> is used for )
the source view and $t$ for the reference view.  $\mathbf{H}_2(\cdot)$ is defined as:

\begin{equation}\label{eq:H2}
%%too long for cvpr paper
%\mathbf{H}_2(f(I_k); d_t, T_{k}, T_{t}, K_{k}, K_{t}) = \mathbf{K}_k \cdot  \mathbf{R}_{k} \cdot \left(\mathcal{I} - \frac{ \mathbf{c}_{k}^{\text{\{t\}}} \cdot \mathbf{n}^{T}_{t}}{d_{t}}\right) \cdot \mathbf{R}^{T}_{t} \cdot \mathbf{K}_{t}^{-1}
\mathbf{H}_2(f(I_k); d_t) = \mathbf{K}_k \cdot  \mathbf{R}_{k} \cdot \left(\mathcal{I} - \frac{ \mathbf{c}_{k}^{\text{\{t\}}} \cdot \mathbf{n}^{T}_{t}}{d_{t}}\right) \cdot \mathbf{R}^{T}_{t} \cdot \mathbf{K}_{t}^{-1}
\end{equation}

\noindent where $\mathcal{I}$ is an identity matrix; $\mathbf{R}_k$ is the rotation matrix for source frame $I_k$; $\mathbf{R}_t$ is the rotation matrix for reference frame $I_t$; $\mathbf{c}_{k}^{\text{\{t\}}}$ is the translation of source camera (for $I_k$) w.r.t. the reference camera (for $I_{\text{t}}$); $\mathbf{n}_{t}$ is the principle axis of the reference camera, and for a fronto-parallel sweep \cite{gallup2007real}, $\mathbf{n}_{t} = [0, 0, 1]^T$. %The intrinsic matrix $\mathbf{K}$ remains constant among different views. 
$\mathbf{H}_2(\cdot)$ is implemented as a backward 2D grid sampling.


The feature extractor $f(\cdot)$ has two variants: i) %one in (one in --> either) 
either D-Net from NRGBD \cite{liu2019neural}, or ii)~ a shallow CNN from MVSNet \cite{yao2018mvsnet}. The former is based on PSMNet \cite{chang2018psmnet}, consisting of four basic residual blocks and spatial pyramid pooling (SPP) for multi-scale feature learning, while the latter is a lightweight structure of seven convolutional layers, each followed by batch normalization (BN) and ReLU, except for the last layer. 
%% Comments by Prof. PM: 
% say that both networks take 5 or N images, compute a cost volume and then depth. This allows us to use either one.

\noindent \textbf{Integrating DPVs over Time.} \,\, The K-Net in NRGBD \cite{liu2019neural} integrates the local estimates of DPVs over time to reduce uncertainty, when processing a video stream. %Let us define $d_t$ as the hidden state, which is the depth (in camera coordinates) at frame $I_t$. The ``belief'' volume $p(d_t|I_{1:t})$ is the conditional distribution of the state giving all the previous frames. 
This integration is implemented as a Bayesian filtering in two iterative steps: \textbf{i)} predicting the DPV for the current frame $I_t$ from history, defined as $p(d_{t-1} | I_{1:t-1}) \rightarrow p(d_{t} | I_{1:t-1})$, and \textbf{ii)} updating the  predicted DPV by integrating a DPV which is estimated from the current local frames $\mathbf{I}_{t-\delta{t}}^{t+\delta{t}}$, defined as $p(d_{t} | I_{1:t-1}) \rightarrow p(d_{t} | I_{1:t})$. Specifically, the prediction step is to warp the previous DPV from the camera coordinate system %(system --> coordinate system)
at $t-1$ to the camera coordinate system at $t$:

\begin{equation}\label{eq:bayesian-prediction}
p(d_{t} | I_{1:t-1}) = \mathbf{H}_3\left( p(d_{t-1} | I_{1:t-1}); T_{t-1}, T_{t}, K_{t-1}, K_{t}\right)
\end{equation} 
\noindent where $T_{t-1}$, $T_{t}$ and $K_{t-1}, K_{t}$ are the camera poses and intrinsics at time $t-1$ and time $t$, and $\mathbf{H}_3(\cdot)$ here is a backward warping operator implemented as 3D grid sampling. Then at current time $t$, the local DPV $p(d_{t} | I_t)$ (omitting $\mathbf{I}_{t-\delta{t}}^{t+\delta{t}}$, $\mathbf{T}_{t-\delta{t}}^{t+\delta{t}}$ and $\mathbf{K}_{t-\delta{t}}^{t+\delta{t}}$ for conciseness in the rest of the %paper
chapter) is computed from the local measurement as in Eq. \ref{eq:dpv}. This local estimate is further used to update the predicted DPV:

\begin{equation}\label{eq:bayesian-update}
p(d_{t} | I_{1:t}) = p(d_{t} | I_{1:t-1}) \cdot p(d_{t} | I_{t})
\end{equation} 
\noindent Please note that the DPV is always normalized in the above equations to ensure $\int_{d_{\text{min}}}^{d_{\text{max}}} p(d) = 1$. By defining $E(d) = \log p(d)$ in logarithm \cite{liu2019neural}, Eq. \ref{eq:bayesian-update} is re-written as

\begin{equation}\label{eq:bayesian-update-log}
E(d_{t} | I_{1:t}) = E(d_{t} | I_{1:t-1}) + E(d_{t} | I_{t})
\end{equation}

\noindent and Eq. \ref{eq:bayesian-update-log} is implemented in an ``adaptive damping'' scheme to update the DPV:

\begin{equation}\label{eq:knet}
E(d_{t} | I_{1:t}) = E(d_{t} | I_{1:t-1}) + g(\Delta E_{t}, I_t)
\end{equation} 

\noindent where $\Delta E_{t} = E(d_{t} | I_{t}) - E(d_{t} | I_{1:t-1})$ is the residual between the measurement and the prediction, and $g(\cdot)$ is the K-Net, which learns to transform the residual $\Delta E_{t}$ into a correction term added back to the prediction.  %Please refer to the appendix for details.

\noindent \textbf{DPV Refinement and Depth Regression.}  \,\,  As in NRGBD \cite{liu2019neural}, the DPV $p(d_t | I_{1:t})$ estimated by K-Net has $1/4$ spatial resolution of the input image, and it is upsampled and refined back to the original image resolution by a network, called R-Net. Here R-Net adopts an encoder-decoder architecture with skip connections, taking as input the low-resolution DPV from the K-Net $g(\cdot)$ and the image features extracted from the feature extractor $f(\cdot)$ in the D-Net, and generating a high-resolution DPV as output. Given the refined DPV $p(d_{t} | I_{t})$, the depth map $\hat{\mathbf{D}}_{t}$ is regressed via the \textit{soft argmin} operator \cite{kendall2017-gcnet} for the reference frame $I_t$:

\begin{equation}\label{eq:softargmin}
%\hat{d} = \sum_{d=0}^{D-1} d \times \sigma(- \mathcal{C}_d)
\hat{\mathbf{D}}_{t} = \sum_{d=d_{\text{min}}}^{d_{\text{max}}} d \cdot p(d_{t} | I_{t})
\end{equation} 

\noindent \textbf{Loss Functions.}  \,\,  Our network is trained end-to-end. For the NRGBD backbone \cite{liu2019neural}, we employ the Negative Log-Likelihood (NLL) loss over the DPV and the ground truth depth $\mathbf{D}_{t}$, i.e., $l_{0} = \text{NLL}(p(d_{t} | I_{t}), \mathbf{D}_{t})$. For the modified backbone with MVSNet \cite{yao2018mvsnet}, we also use $L_1$ loss between the predicted depth map $\hat{\mathbf{D}}_{t}$ and the ground truth depth $\mathbf{D}_{t}$, i.e., $l_{1} = \| \hat{\mathbf{D}}_{t} - \mathbf{D}_{t} \|_{1}$. Therefore, the total loss is a weighted sum as $l = \lambda_0 l_0 + \lambda_1 l_1$.

%% Comments by Prof. PM:
% we need to discuss how losses perform at the end

\begin{figure*}%[!htbp]
    \centering
    \renewcommand{\tabcolsep}{1pt}
    \scriptsize
    \includegraphics[width=\textwidth]{ imgs-\imgres/our-archi-01.png}
    \caption{\textbf{Architecture of our method.} Our framework extends the backbone network by incorporating Gaussian modulation \cite{Poggi_guided_stereo_CVPR_2019} from depth-guidance and dynamic filtering \cite{jia2016dynamic} to adaptively reason about the past for current DPV prediction when processing video streams.}
    \label{mvs-fig:archi-ours}
    %\vspace{-8pt}
\end{figure*}

%\ccjscomments{Need to discuss how losses perform at the end???}


\subsection{Depth-Guided DPV Integration}\label{depth-guided-dpv-update}


Here we present our framework that extends the backbone network by incorporating Gaussian modulation from depth-guidance and dynamic filtering to adaptively reason about the past for current DPV prediction when processing video streams. Essentially, we include a depth-guided Gaussian modulation layer \cite{Poggi_guided_stereo_CVPR_2019} and a Dynamic Filtering Network (DFN) layer \cite{jia2016dynamic} to the backbone NRGBD \cite{liu2019neural} to model the spatio-temporal relations, \cf Fig. \ref{mvs-fig:archi-ours}.

\noindent \textbf{Depth-Guided Gaussian Modulation.} \,\, Instead of predicting the DPV by warping from the camera coordinate system at time $t-1$ to the camera coordinate system at time $t$, we propose to warp the \textit{depth} map from $t-1$ to $t$. 
%%
%% Please note that the warping of DPVs requires 3D grid sampling at $O(H \times W \times D)$ (H: image height, W: image width, and D: the number of discrete depth values) time and space cost, while our depth-warping requires %bilinear interpolation %(bilinear interpolation --> 2D grid sampling ---- even though this is not  100% accurate since the Gaussians cover multiple voxels. How many voxels does a Gaussian cover?) 2D grid sampling with $O(H\times W)$ cost, \ccjscomments{??? Q: How many voxels does a Gaussian cover? A: One Gaussain affects one pixel $(u,v)$ for all the $d \in [d_{min}, d_{max}]$. The depth warping itself does be O(WH). But to generate a DPV from depth, it is inevitable to be $O(WHD)$. Here we want to emphasize the depth warping O(WH) vs the direct volume warping O(HWD)} enabling efficient and online deployment.
%% Comments by Porf. PM: "delete  -- We need to explain why warping depth works better. In my experience, warping the volume leads to blurring and potentially amplifies noise by warping local cost minima that were correctly not selected as the depth at t-1. The problem is that we don't have evidence for this, so let's not write it yet."
Based on the warped depth guidance, we extend the feature enhancement technique by a Gaussian filter \cite{Poggi_guided_stereo_CVPR_2019} to modulate the local measurement of DPV $p(d_t | I_t)$ at time $t$, via \textit{amplifying} the probability related to the hypotheses suggested by these warped depth hints and \textit{dampening} the remaining ones, as shown in Figure \ref{mvs-fig:guided_stereo}. Specifically, the predicted DPV $p(d_{t} | I_{1:t-1})$, represented by a Gaussian modulating function $h(\cdot)$, is defined as

\begin{equation}\label{eq:gaussian}
p(d_{t} | I_{1:t-1}) = h(\bar{d}; \Tilde{d}_t, k, c) = k \cdot e^{- \frac{(\bar{d} - \Tilde{d}_t)^2}{2c^2} }
\end{equation} 

\noindent where $\bar{d}$ is a depth hypothesis uniformly sampled over the range $[d_{\text{min}},d_{\text{max}}]$, $k$ and $c$ represent the magnitude and the width of the Gaussian, and the warped depth hint $\Tilde{d}_t$ is obtained by: 

\begin{equation}\label{eq:depth-warping}
\Tilde{d}_t = \mathbf{H}_2\left( d_{t-1}; I_{t-1}, I_{t}, T_{t-1}, T_{t}, K_{t-1}, K_{t}\right)
\end{equation} 

\noindent where $\mathbf{H}_2(\cdot)$ is a 2D homography obtained by setting the source frame index $k$ in Eq. \ref{eq:H2} as $k = t-1$. Image frames $I_{t-1}$ and $I_{t}$, and camera poses $T_{t-1}$, $T_{t}$ and intrinsics $K_{t-1}$, $K_{t}$ correspond to time $t-1$ and time $t$, respectively. Here $\mathbf{H}_2(\cdot)$ is implemented as a forward 2D grid sampling. 

Thus, to obtain a new integrated prediction of DPV $p(d_{t} | I_{1:t-1})$ via multiplying the local DPV $p(d_{t} | I_{t})$ by the modulating function $h(\cdot)$, we apply

\begin{equation}\label{eq:depth-warping-dpv}
p(d_{t} | I_{1:t}) = \left(  1 - v_t + v_t \cdot k \cdot e^{- \frac{(\bar{d} - \Tilde{d}_t)^2}{2c^2} } \right) \cdot p(d_{t} | I_{t})
\end{equation} 

\noindent where $v_t$ is a binary mask, specifying which elements of the depth guidance $\Tilde{d}_t$ are valid, i.e., $v_t(u,v) = 1$ being valid if $d_{\text{min}} \leq \Tilde{d}_t(u, v) \leq d_{\text{max}}$ for a pixel $(u,v)$, otherwise $v_t(u,v) = 0$.

\noindent Again, by introducing the logarithm $E(d) = \log p(d)$ \cite{liu2019neural}, Eq. \ref{eq:depth-warping-dpv} is re-written as 

\begin{equation}\label{eq:depth-warping-dpv-log}
E(d_{t} | I_{1:t}) = v_t \cdot \left(  \log{k} - \frac{(\bar{d} - \Tilde{d}_t)^2}{2c^2} \right) +  E(d_{t} | I_{t})
\end{equation}


\noindent As for the hyper-parameters $k$ and $c$, we adopt two schemes: i) \textit{global}, where constant values (e.g., $k=10$ and $c=10$) are used, and ii) \textit{dynamic}, where a DFN is employed to dynamically generate $k$ and $c$ for each spatial location. %see details in the following.

\begin{figure*}[t]
    \centering
    \renewcommand{\tabcolsep}{1pt}
    \scriptsize
    \includegraphics[width=1.0\textwidth]{ imgs-\imgres/guided-stereo.png} 
    \caption{\textbf{Illustration of the Gaussian feature enhancement from \cite{Poggi_guided_stereo_CVPR_2019}.} In blue, features $\mathcal{F}$ for pixel $i$, $j$ in proximity of depth $d= g_{ij}$, in black the modulating function, in red enhanced valid features $\mathcal{G}$ with binary mask value $v_{ij} = 1$, applied to correlation features (left) or dissimilarity functions (right).
    }
    \label{mvs-fig:guided_stereo}
\end{figure*}


\noindent \textbf{Dynamic Gaussian Modulation.} \,\, We employ a lightweight DFN \cite{jia2016dynamic}, by taking as input the confidence $p^w_{t}$, which is obtained by warping the winning probability, i.e., $p^w_{t} = \mathbf{H}_2(\text{max}_{d}( p(d_{t-1}| I_{t-1})))$, the image RGB intensity of $I_t$ and its corresponding deep features $f(I_t)$. This way, the DFN can dynamically generate distinctive values of $k$ and $c$ for different spatial positions with varying input contents, see the top branch in Fig. \ref{mvs-fig:archi-ours}. When generating the Gaussian parameters $k$ and $c$, we compare two variants of DFN networks: i)~ {\myqcrfont DFN-I}, which is depth channel independent, with $k$ and $c$ %having the size $1 \times H \times W$ per pixel, 
per pixel with dimensions equal to $1 \times H \times W$, and ii) {\myqcrfont DFN-A}, which is depth channel aware, with $k$ and $c$ %having the size $D \times H \times W$ per pixel and per depth.
per pixel and per depth with dimensions equal to $D \times H \times W$. These two variants are evaluated in Sec. \ref{dg-mvsnet:experiment}.

%\begin{figure*}[t]
%    \centering
%    \renewcommand{\tabcolsep}{1pt}
%    \scriptsize
%    \includegraphics[width=0.6\textwidth]{ imgs-low-res/dfn-tmp.png} 
%    \caption{\textbf{\ccjscomments{To Change Figure ???}} DFN Gaussian ???
%    }
%    \label{mvs-fig:dfn-gaussian}
%\end{figure*}

==> fig-dtu.tex <==
\begin{figure*}[t]
    \centering
    \renewcommand{\tabcolsep}{0.2pt}
    \scriptsize
    \begin{tabular}{ccccc}
      \includegraphics[width=0.2\textwidth]{qualitatives/dtu-img_00000000.png} &  \includegraphics[width=0.2\textwidth]{qualitatives/dtu-d_gt_clr_00000000.png} & 
        \includegraphics[width=0.2\textwidth]{qualitatives/iter-dtu-d_clr_00000000.png} & \includegraphics[width=0.2\textwidth]{qualitatives/pair-dtu-d_clr_00000000.png} &
        \includegraphics[width=0.2\textwidth]{qualitatives/our-dtu-d_clr_00000000.png} \\
        
        \includegraphics[width=0.2\textwidth]{qualitatives/dtu-img_00000001.png} &  \includegraphics[width=0.2\textwidth]{qualitatives/dtu-d_gt_clr_00000001.png} & 
        \includegraphics[width=0.2\textwidth]{qualitatives/iter-dtu-d_clr_00000001.png} & \includegraphics[width=0.2\textwidth]{qualitatives/pair-dtu-d_clr_00000001.png} &
        \includegraphics[width=0.2\textwidth]{qualitatives/our-dtu-d_clr_00000001.png} \\
        
        \includegraphics[width=0.2\textwidth]{qualitatives/dtu-img_00000002.png} &  \includegraphics[width=0.2\textwidth]{qualitatives/dtu-d_gt_clr_00000002.png} & 
        \includegraphics[width=0.2\textwidth]{qualitatives/iter-dtu-d_clr_00000002.png} & \includegraphics[width=0.2\textwidth]{qualitatives/pair-dtu-d_clr_00000002.png} &
        \includegraphics[width=0.2\textwidth]{qualitatives/our-dtu-d_clr_00000002.png} \\
        
        %%%%% scene 2 %%%%%%%
        \includegraphics[width=0.2\textwidth]{qualitatives/dtu-img_00000400.png.jpg} &  \includegraphics[width=0.2\textwidth]{qualitatives/dtu-d_gt_clr_00000400.png} & 
        \includegraphics[width=0.2\textwidth]{qualitatives/iter-dtu-d_clr_00000400.png} & \includegraphics[width=0.2\textwidth]{qualitatives/pair-dtu-d_clr_00000400.png} &
        \includegraphics[width=0.2\textwidth]{qualitatives/our-dtu-d_clr_00000400.png} \\
        \includegraphics[width=0.2\textwidth]{qualitatives/dtu-img_00000401.jpg} &  \includegraphics[width=0.2\textwidth]{qualitatives/dtu-d_gt_clr_00000401.png} & 
        \includegraphics[width=0.2\textwidth]{qualitatives/iter-dtu-d_clr_00000401.png} & \includegraphics[width=0.2\textwidth]{qualitatives/pair-dtu-d_clr_00000401.png} &
        \includegraphics[width=0.2\textwidth]{qualitatives/our-dtu-d_clr_00000401.png} \\
        \includegraphics[width=0.2\textwidth]{qualitatives/dtu-img_00000403.jpg} &  \includegraphics[width=0.2\textwidth]{qualitatives/dtu-d_gt_clr_00000403.png} & 
        \includegraphics[width=0.2\textwidth]{qualitatives/iter-dtu-d_clr_00000403.png} & \includegraphics[width=0.2\textwidth]{qualitatives/pair-dtu-d_clr_00000403.png} &
        \includegraphics[width=0.2\textwidth]{qualitatives/our-dtu-d_clr_00000403.png} \\
        
        %%%%% scene 3 %%%%%%%
        \includegraphics[width=0.2\textwidth]{qualitatives/dtu-img_00000800.jpg} &  \includegraphics[width=0.2\textwidth]{qualitatives/dtu-d_gt_clr_00000800.png} & 
        \includegraphics[width=0.2\textwidth]{qualitatives/iter-dtu-d_clr_00000800.png} & \includegraphics[width=0.2\textwidth]{qualitatives/pair-dtu-d_clr_00000800.png} &
        \includegraphics[width=0.2\textwidth]{qualitatives/our-dtu-d_clr_00000800.png} \\
        \includegraphics[width=0.2\textwidth]{qualitatives/dtu-img_00000803.jpg} &  \includegraphics[width=0.2\textwidth]{qualitatives/dtu-d_gt_clr_00000803.png} & 
        \includegraphics[width=0.2\textwidth]{qualitatives/iter-dtu-d_clr_00000803.png} & \includegraphics[width=0.2\textwidth]{qualitatives/pair-dtu-d_clr_00000803.png} &
        \includegraphics[width=0.2\textwidth]{qualitatives/our-dtu-d_clr_00000803.png} \\
        
        %\normalsize (a) & \normalsize (b) & \normalsize (c) & \normalsize (d) & \normalsize (e)\\
        \normalsize Ref & \normalsize GT & \normalsize IterMVS & \normalsize PairNet & \normalsize Ours\\
    \end{tabular}
    \vspace{-2pt}
    \caption{Qualitative results on DTU \cite{dtu_jensen2014large}. Columns from left to right show reference image, ground truth depth, and the estimated depth for baseline IterMVS \cite{itermvs_wang2021}, PairNet \cite{deepvideomvs2021} and our method, respectively. %Our method outperforms IterMVS visibly, and on par with PairNet. 
    }
    \label{fig:qualitatives_dtu}
\end{figure*}

==> fig-scannet.tex <==
\begin{figure*}[t]
    \centering
    \renewcommand{\tabcolsep}{0.2pt}
    \scriptsize
    \begin{tabular}{ccccc}
    %%%%%%%%%%%%%%
    % sample 1: scene0707_00/frames/color/000038.png
    %%%%%%%%%%%%%%
      \includegraphics[width=0.2\textwidth]{qualitatives/scannet-img_00000002.png} &  
      
     \includegraphics[width=0.2\textwidth]{qualitatives/scannetd_gt_clr_00000002.png} & 
     
     \begin{overpic}[width=0.2\textwidth]{qualitatives/iter-scannet-d_clr_00000002.png}
        %\put (72,65) {$\displaystyle\textcolor{white}{\textbf{0.0557}}$}
        \put(56,32){{\color{red} \circle{30}}}
        \end{overpic} &
      \begin{overpic}[width=0.2\textwidth]{qualitatives/pair-scannet-d_clr_00000002.png}
      %\put (72,65) {$\displaystyle\textcolor{white}{\textbf{0.0355}}$}
      \put(56,32){{\color{red} \circle{30}}}
      \end{overpic} &
      \begin{overpic}[width=0.2\textwidth]{qualitatives/our-scannet-d_clr_00000002.png} 
      %\put (72,65) {$\displaystyle\textcolor{white}{\textbf{0.0333}}$}
      \put(56,32){{\color{green} \circle{30}}}
      \end{overpic} \\
    
    %%%%%%%%%%%%%%
    % sample 2: scene0712_00/frames/color/003905.png
    %%%%%%%%%%%%%%
        \includegraphics[width=0.2\textwidth]{qualitatives/scannet-img_00006371.png} &  \includegraphics[width=0.2\textwidth]{qualitatives/scannetd_gt_clr_00006371.png} & 
        \begin{overpic}[width=0.2\textwidth]{qualitatives/iter-scannet-d_clr_00006371.png}
        %\put (5,65) {$\displaystyle\textcolor{white}{\textbf{0.1471}}$}
        \put(56,40){{\color{red} \circle{40}}}
        \end{overpic} &
      \begin{overpic}[width=0.2\textwidth]{qualitatives/pair-scannet-d_clr_00006371.png}
      %\put (5,65) {$\displaystyle\textcolor{white}{\textbf{0.0997}}$}
      \put(56,40){{\color{red} \circle{40}}}
      \end{overpic} &
      \begin{overpic}[width=0.2\textwidth]{qualitatives/our-scannet-d_clr_00006371.png} 
      %\put (5,65){$\displaystyle\textcolor{white}{\textbf{0.0833}}$}
      \put(56,40){{\color{green} \circle{40}}}
      \end{overpic} \\
    		


    %%%%%%%%%%%%%%
    % sample 3: scene0776_00/frames/color/002062.png
    %%%%%%%%%%%%%%
        \includegraphics[width=0.2\textwidth]{qualitatives/scannet-img_00019111.png} &  \includegraphics[width=0.2\textwidth]{qualitatives/scannetd_gt_clr_00019111.png} & 
        \begin{overpic}[width=0.2\textwidth]{qualitatives/iter-scannet-d_clr_00019111.png}
        %\put (72,65){$\displaystyle\textcolor{white}{\textbf{0.0592}}$}
        \put(46,70){{\color{red} \circle{20}}}
        \put(65,35){{\color{red} \circle{30}}}
        \end{overpic} &
      \begin{overpic}[width=0.2\textwidth]{qualitatives/pair-scannet-d_clr_00019111.png}
      %\put (72,65){$\displaystyle\textcolor{white}{\textbf{0.0573}}$}
      \put(46,70){{\color{red} \circle{20}}}
      \put(65,35){{\color{red} \circle{30}}}
      \end{overpic} &
      \begin{overpic}[width=0.2\textwidth]{qualitatives/our-scannet-d_clr_00019111.png} 
      %\put (72,65){$\displaystyle\textcolor{white}{\textbf{0.0528}}$}
      \put(46,70){{\color{green} \circle{20}}}
      \put(65,35){{\color{green} \circle{30}}}
      \end{overpic} \\
    
    
    %%%%%%%%%%%%%%
    % sample 4:scene0806_00/frames/color/001097.png 
    %%%%%%%%%%%%%%
      \includegraphics[width=0.2\textwidth]{qualitatives/scannet-img_00025474.png} &  \includegraphics[width=0.2\textwidth]{qualitatives/scannetd_gt_clr_00025474.png} &
        \begin{overpic}[width=0.2\textwidth]{qualitatives/iter-scannet-d_clr_00025474.png}
        %\put (5,65){$\displaystyle\textcolor{white}{\textbf{0.0721}}$}
        \put(65,70){{\color{red} \circle{20}}}
        \put(65,40){{\color{red} \circle{30}}}
        \end{overpic} &
      \begin{overpic}[width=0.2\textwidth]{qualitatives/pair-scannet-d_clr_00025474.png}
      %\put (5,65){$\displaystyle\textcolor{white}{\textbf{0.0593}}$}
      \put(65,70){{\color{red} \circle{20}}}
      \put(65,40){{\color{red} \circle{30}}}
      \end{overpic} &
      \begin{overpic}[width=0.2\textwidth]{qualitatives/our-scannet-d_clr_00025474.png} 
      %\put (5,65){$\displaystyle\textcolor{white}{\textbf{0.0652}}$}
      \put(65,70){{\color{green} \circle{20}}}
      \put(65,40){{\color{green} \circle{30}}}
      \end{overpic} \\
      
        \normalsize Ref. image & \normalsize GR depth & \normalsize IterMVS & \normalsize PairNet & \normalsize Ours \\
    \end{tabular}
    \vspace{-2pt}
    \caption{Qualitative results on ScanNet \cite{dai2017scannet} test set. Left two columns show reference image and ground truth depth, and other columns are the estimated depth by baseline IterMVS \cite{itermvs_wang2021}, PairNet \cite{deepvideomvs2021} and ours (the full version), respectively. Our method outperform the baselines on thin structures, small objects and boundaries, as highlighted in {\color{green} green} for ours and in {\color{red} red} for the baselines.
    }
    \label{fig:qualitatives_scannet}
\end{figure*}

